Computing volume fractions and signed distances from triangulated surfaces immersed in unstructured meshes

Available algorithms for the initialization of volume fractions typically utilize exact functions to model fluid interfaces, or they rely on computationally costly intersections between volume meshes. Here, a new algorithm is proposed that computes signed distances and volume fractions on unstructured meshes from arbitrarily shaped surfaces, e.g. originating from experimental data. The proposed algorithm calculates signed distances geometrically near the fluid interface, approximated as a triangle surface mesh, and propagates the inside/outside information by an approximate solution of a Laplace equation. Volume fractions are computed based on signed distances, using either geometrical intersections between cells of the unstructured mesh and a sub-set of the surface mesh that represents the interface, or using a polynomial approximation and adaptive mesh refinement. Although primarily developed for multiphase flow simulations, the proposed algorithm can potentially be used for other problems that require a phase-indicator: inside/outside information with respect to an arbitrarily shaped surface on arbitrarily unstructured meshes.

==> credit-statement.tex <==
\section*{CRediT author statement}

\begin{description}

\item Tobias Tolle: Conceptualization, Methodology, Software, Validation, Investigation, Writing - Original Draft, Writing - Review \& Editing, Visualization 

\item Dirk Gr\"unding: Conceptualization, Software, Formal analysis, Data Curation, Writing - Original Draft, Writing - Review \& Editing, Visualization 

\item Dieter Bothe: Writing - Review \& Editing, Supervision, Funding acquisition

\item Tomislav Mari\'c: Conceptualization, Methodology, Software, Validation, Investigation, Data Curation, Writing - Original Draft, Writing - Review \& Editing, Visualization, Supervision, Project administration, Funding acquisition

\end{description}


==> data/Data_Pandas_Dframe-equidistant_ellipsoid-SMCA.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  MAX\_REFINEMENT\_LEVEL &  N\_TRIANGLES\_ROOT &    N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &         1168 &                     0.099210 &                      0.099461 &                            0.002525 &                 163107 &                     1 &         34.176015 &   16.0 &                        0.013138 &          0.163107 \\
   32768 &         1168 &                     0.099243 &                      0.099461 &                            0.002193 &                 312504 &                     0 &         34.176015 &   32.0 &                        0.012810 &          0.312504 \\
  262144 &         1168 &                     0.099408 &                      0.099461 &                            0.000532 &                1176141 &                     0 &         34.176015 &   64.0 &                        0.011167 &          1.176141 \\
 2097152 &         1168 &                     0.099448 &                      0.099461 &                            0.000132 &                6799602 &                     0 &         34.176015 &  128.0 &                        0.010771 &          6.799602 \\
    4096 &         7032 &                     0.100292 &                      0.100354 &                            0.000621 &                 863516 &                     2 &         83.857021 &   16.0 &                        0.002381 &          0.863516 \\
   32768 &         7032 &                     0.100292 &                      0.100354 &                            0.000622 &                 929228 &                     1 &         83.857021 &   32.0 &                        0.002381 &          0.929228 \\
  262144 &         7032 &                     0.100301 &                      0.100354 &                            0.000531 &                1847491 &                     0 &         83.857021 &   64.0 &                        0.002290 &          1.847491 \\
 2097152 &         7032 &                     0.100340 &                      0.100354 &                            0.000141 &                8230583 &                     0 &         83.857021 &  128.0 &                        0.001902 &          8.230583 \\
    4096 &        27256 &                     0.100471 &                      0.100487 &                            0.000163 &                3449974 &                     3 &        165.093913 &   16.0 &                        0.000599 &          3.449974 \\
   32768 &        27256 &                     0.100471 &                      0.100487 &                            0.000159 &                3637844 &                     2 &        165.093913 &   32.0 &                        0.000595 &          3.637844 \\
  262144 &        27256 &                     0.100471 &                      0.100487 &                            0.000157 &                4193769 &                     1 &        165.093913 &   64.0 &                        0.000593 &          4.193769 \\
 2097152 &        27256 &                     0.100473 &                      0.100487 &                            0.000143 &               10892967 &                     0 &        165.093913 &  128.0 &                        0.000579 &         10.892967 \\
    4096 &       106624 &                     0.100517 &                      0.100522 &                            0.000042 &               14512448 &                     4 &        326.533306 &   16.0 &                        0.000135 &         14.512448 \\
   32768 &       106624 &                     0.100517 &                      0.100522 &                            0.000041 &               13699459 &                     3 &        326.533306 &   32.0 &                        0.000134 &         13.699459 \\
  262144 &       106624 &                     0.100518 &                      0.100522 &                            0.000040 &               15708862 &                     2 &        326.533306 &   64.0 &                        0.000133 &         15.708862 \\
 2097152 &       106624 &                     0.100518 &                      0.100522 &                            0.000040 &               22151811 &                     1 &        326.533306 &  128.0 &                        0.000133 &         22.151811 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-equidistant_ellipsoid-SMCI.tex <==
\begin{tabular}{rrrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  N\_TRIANGLES\_PER\_CELL &  N\_INTERSECTED\_CELLS &  N\_TRIANGLES\_ROOT &    N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &         1168 &                     0.099447 &                      0.099461 &                            0.000139 &                 209027 &            129.942308 &                  416 &         34.176015 &   16.0 &                        0.010778 &          0.209027 \\
   32768 &         1168 &                     0.099456 &                      0.099461 &                            0.000056 &                 479516 &             59.765550 &                 1672 &         34.176015 &   32.0 &                        0.010696 &          0.479516 \\
  262144 &         1168 &                     0.099459 &                      0.099461 &                            0.000020 &                1450333 &             34.418577 &                 6632 &         34.176015 &   64.0 &                        0.010660 &          1.450333 \\
 2097152 &         1168 &                     0.099461 &                      0.099461 &                            0.000005 &                6529869 &             23.545345 &                26640 &         34.176015 &  128.0 &                        0.010646 &          6.529869 \\
    4096 &         7032 &                     0.100351 &                      0.100354 &                            0.000027 &                 626191 &            463.153846 &                  416 &         83.857021 &   16.0 &                        0.001787 &          0.626191 \\
   32768 &         7032 &                     0.100351 &                      0.100354 &                            0.000025 &                1094848 &            166.181818 &                 1672 &         83.857021 &   32.0 &                        0.001785 &          1.094848 \\
  262144 &         7032 &                     0.100353 &                      0.100354 &                            0.000014 &                2530450 &             73.361011 &                 6648 &         83.857021 &   64.0 &                        0.001774 &          2.530450 \\
 2097152 &         7032 &                     0.100354 &                      0.100354 &                            0.000004 &                8733452 &             39.058577 &                26768 &         83.857021 &  128.0 &                        0.001765 &          8.733452 \\
    4096 &        27256 &                     0.100487 &                      0.100487 &                            0.000006 &                2011276 &           1445.826923 &                  416 &        165.093913 &   16.0 &                        0.000442 &          2.011276 \\
   32768 &        27256 &                     0.100487 &                      0.100487 &                            0.000006 &                2666170 &            447.732057 &                 1672 &        165.093913 &   32.0 &                        0.000442 &          2.666170 \\
  262144 &        27256 &                     0.100487 &                      0.100487 &                            0.000005 &                4835306 &            163.181709 &                 6648 &        165.093913 &   64.0 &                        0.000441 &          4.835306 \\
 2097152 &        27256 &                     0.100487 &                      0.100487 &                            0.000003 &               12766619 &             70.930087 &                26776 &        165.093913 &  128.0 &                        0.000439 &         12.766619 \\
    4096 &       106624 &                     0.100521 &                      0.100522 &                            0.000002 &                9601813 &           4974.076923 &                  416 &        326.533306 &   16.0 &                        0.000095 &          9.601813 \\
   32768 &       106624 &                     0.100521 &                      0.100522 &                            0.000002 &                8289723 &           1394.545455 &                 1672 &        326.533306 &   32.0 &                        0.000095 &          8.289723 \\
  262144 &       106624 &                     0.100521 &                      0.100522 &                            0.000002 &               11371037 &            438.035499 &                 6648 &        326.533306 &   64.0 &                        0.000095 &         11.371037 \\
 2097152 &       106624 &                     0.100521 &                      0.100522 &                            0.000002 &               23301370 &            158.252838 &                26776 &        326.533306 &  128.0 &                        0.000095 &         23.301370 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-equidistant_sphere-SMCA.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  MAX\_REFINEMENT\_LEVEL &  N\_TRIANGLES\_ROOT &    N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &          356 &                     0.013582 &                      0.013691 &                            0.007924 &                  60192 &                     1 &         18.867962 &   16.0 &                        0.039240 &          0.060192 \\
   32768 &          356 &                     0.013596 &                      0.013691 &                            0.006902 &                 133878 &                     0 &         18.867962 &   32.0 &                        0.038251 &          0.133878 \\
  262144 &          356 &                     0.013665 &                      0.013691 &                            0.001880 &                 737747 &                     0 &         18.867962 &   64.0 &                        0.033386 &          0.737747 \\
 2097152 &          356 &                     0.013685 &                      0.013691 &                            0.000435 &                5483932 &                     0 &         18.867962 &  128.0 &                        0.031988 &          5.483932 \\
    4096 &         1824 &                     0.014019 &                      0.014050 &                            0.002227 &                 241551 &                     2 &         42.708313 &   16.0 &                        0.008362 &          0.241551 \\
   32768 &         1824 &                     0.014021 &                      0.014050 &                            0.002112 &                 264196 &                     1 &         42.708313 &   32.0 &                        0.008248 &          0.264196 \\
  262144 &         1824 &                     0.014025 &                      0.014050 &                            0.001803 &                 871407 &                     0 &         42.708313 &   64.0 &                        0.007941 &          0.871407 \\
 2097152 &         1824 &                     0.014043 &                      0.014050 &                            0.000492 &                5750931 &                     0 &         42.708313 &  128.0 &                        0.006637 &          5.750931 \\
    4096 &         7132 &                     0.014107 &                      0.014115 &                            0.000575 &                 959514 &                     3 &         84.451169 &   16.0 &                        0.002132 &          0.959514 \\
   32768 &         7132 &                     0.014108 &                      0.014115 &                            0.000525 &                 917911 &                     2 &         84.451169 &   32.0 &                        0.002082 &          0.917911 \\
  262144 &         7132 &                     0.014107 &                      0.014115 &                            0.000543 &                1451334 &                     1 &         84.451169 &   64.0 &                        0.002100 &          1.451334 \\
 2097152 &         7132 &                     0.014108 &                      0.014115 &                            0.000491 &                6348671 &                     0 &         84.451169 &  128.0 &                        0.002049 &          6.348671 \\
    4096 &        28160 &                     0.014130 &                      0.014132 &                            0.000147 &                3832615 &                     4 &        167.809416 &   16.0 &                        0.000540 &          3.832615 \\
   32768 &        28160 &                     0.014130 &                      0.014132 &                            0.000137 &                3474960 &                     3 &        167.809416 &   32.0 &                        0.000530 &          3.474960 \\
  262144 &        28160 &                     0.014130 &                      0.014132 &                            0.000137 &                4250605 &                     2 &        167.809416 &   64.0 &                        0.000530 &          4.250605 \\
 2097152 &        28160 &                     0.014130 &                      0.014132 &                            0.000138 &                8788266 &                     1 &        167.809416 &  128.0 &                        0.000531 &          8.788266 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-equidistant_sphere-SMCI.tex <==
\begin{tabular}{rrrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  N\_TRIANGLES\_PER\_CELL &  N\_INTERSECTED\_CELLS &  N\_TRIANGLES\_ROOT &    N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &          356 &                     0.013691 &                      0.013691 &                        4.327694e-06 &                  65564 &            127.851562 &                  128 &         18.867962 &   16.0 &                        0.031570 &          0.065564 \\
   32768 &          356 &                     0.013691 &                      0.013691 &                        2.934645e-06 &                 166704 &             68.375000 &                  416 &         18.867962 &   32.0 &                        0.031569 &          0.166704 \\
  262144 &          356 &                     0.013691 &                      0.013691 &                        9.400489e-07 &                 693843 &             35.171023 &                 1760 &         18.867962 &   64.0 &                        0.031567 &          0.693843 \\
 2097152 &          356 &                     0.013691 &                      0.013691 &                        3.500448e-07 &                4318320 &             24.497509 &                 6824 &         18.867962 &  128.0 &                        0.031567 &          4.318320 \\
    4096 &         1824 &                     0.014050 &                      0.014050 &                        9.877262e-16 &                 170083 &            413.554688 &                  128 &         42.708313 &   16.0 &                        0.006149 &          0.170083 \\
   32768 &         1824 &                     0.014050 &                      0.014050 &                        2.592781e-15 &                 315990 &            168.079327 &                  416 &         42.708313 &   32.0 &                        0.006149 &          0.315990 \\
  262144 &         1824 &                     0.014050 &                      0.014050 &                        2.716247e-15 &                 958566 &             71.840341 &                 1760 &         42.708313 &   64.0 &                        0.006149 &          0.958566 \\
 2097152 &         1824 &                     0.014050 &                      0.014050 &                        3.950905e-15 &                4769002 &             39.063439 &                 6920 &         42.708313 &  128.0 &                        0.006149 &          4.769002 \\
    4096 &         7132 &                     0.014115 &                      0.014115 &                        4.092506e-14 &                 520912 &           1295.289062 &                  128 &         84.451169 &   16.0 &                        0.001558 &          0.520912 \\
   32768 &         7132 &                     0.014115 &                      0.014115 &                        1.720573e-15 &                 689828 &            462.483173 &                  416 &         84.451169 &   32.0 &                        0.001558 &          0.689828 \\
  262144 &         7132 &                     0.014115 &                      0.014115 &                        1.216691e-14 &                1516350 &            162.683523 &                 1760 &         84.451169 &   64.0 &                        0.001558 &          1.516350 \\
 2097152 &         7132 &                     0.014115 &                      0.014115 &                        3.367408e-14 &                5799068 &             72.250289 &                 6920 &         84.451169 &  128.0 &                        0.001558 &          5.799068 \\
    4096 &        28160 &                     0.014132 &                      0.014132 &                        1.344092e-10 &                2554149 &           4501.882812 &                  128 &        167.809416 &   16.0 &                        0.000393 &          2.554149 \\
   32768 &        28160 &                     0.014132 &                      0.014132 &                        1.344773e-10 &                2132074 &           1465.235577 &                  416 &        167.809416 &   32.0 &                        0.000393 &          2.132074 \\
  262144 &        28160 &                     0.014132 &                      0.014132 &                        1.345436e-10 &                3122986 &            443.196023 &                 1760 &        167.809416 &   64.0 &                        0.000393 &          3.122986 \\
 2097152 &        28160 &                     0.014132 &                      0.014132 &                        1.345607e-10 &                8199635 &            162.719653 &                 6920 &        167.809416 &  128.0 &                        0.000393 &          8.199635 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-perturbed_alpha_0.25_ellipsoid-SMCA.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  MAX\_REFINEMENT\_LEVEL &  N\_TRIANGLES\_ROOT &    N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &         1168 &                     0.099200 &                      0.099461 &                            0.002626 &                 176118 &                     1 &         34.176015 &   16.0 &                        0.013238 &          0.176118 \\
   32768 &         1168 &                     0.099222 &                      0.099461 &                            0.002405 &                 318078 &                     0 &         34.176015 &   32.0 &                        0.013020 &          0.318078 \\
  262144 &         1168 &                     0.099401 &                      0.099461 &                            0.000607 &                1115884 &                     0 &         34.176015 &   64.0 &                        0.011241 &          1.115884 \\
 2097152 &         1168 &                     0.099447 &                      0.099461 &                            0.000148 &                6188386 &                     0 &         34.176015 &  128.0 &                        0.010787 &          6.188386 \\
    4096 &         7032 &                     0.100289 &                      0.100354 &                            0.000643 &                 886815 &                     2 &         83.857021 &   16.0 &                        0.002402 &          0.886815 \\
   32768 &         7032 &                     0.100289 &                      0.100354 &                            0.000644 &                 981061 &                     1 &         83.857021 &   32.0 &                        0.002403 &          0.981061 \\
  262144 &         7032 &                     0.100295 &                      0.100354 &                            0.000591 &                1818094 &                     0 &         83.857021 &   64.0 &                        0.002350 &          1.818094 \\
 2097152 &         7032 &                     0.100339 &                      0.100354 &                            0.000149 &                7893929 &                     0 &         83.857021 &  128.0 &                        0.001909 &          7.893929 \\
    4096 &        27256 &                     0.100471 &                      0.100487 &                            0.000161 &                3468107 &                     3 &        165.093913 &   16.0 &                        0.000597 &          3.468107 \\
   32768 &        27256 &                     0.100471 &                      0.100487 &                            0.000159 &                3714366 &                     2 &        165.093913 &   32.0 &                        0.000595 &          3.714366 \\
  262144 &        27256 &                     0.100471 &                      0.100487 &                            0.000160 &                4399784 &                     1 &        165.093913 &   64.0 &                        0.000596 &          4.399784 \\
 2097152 &        27256 &                     0.100472 &                      0.100487 &                            0.000150 &               10566517 &                     0 &        165.093913 &  128.0 &                        0.000585 &         10.566517 \\
    4096 &       106624 &                     0.100518 &                      0.100522 &                            0.000040 &               13856502 &                     4 &        326.533306 &   16.0 &                        0.000133 &         13.856502 \\
   32768 &       106624 &                     0.100518 &                      0.100522 &                            0.000040 &               13992048 &                     4 &        326.533306 &   32.0 &                        0.000133 &         13.992048 \\
  262144 &       106624 &                     0.100518 &                      0.100522 &                            0.000040 &               15885896 &                     2 &        326.533306 &   64.0 &                        0.000133 &         15.885896 \\
 2097152 &       106624 &                     0.100518 &                      0.100522 &                            0.000040 &               24583933 &                     2 &        326.533306 &  128.0 &                        0.000133 &         24.583933 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-perturbed_alpha_0.25_sphere-SMCA.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  MAX\_REFINEMENT\_LEVEL &  N\_TRIANGLES\_ROOT &    N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &          356 &                     0.013565 &                      0.013691 &                            0.009233 &                  59664 &                     1 &         18.867962 &   16.0 &                        0.040508 &          0.059664 \\
   32768 &          356 &                     0.013578 &                      0.013691 &                            0.008217 &                 133140 &                     0 &         18.867962 &   32.0 &                        0.039524 &          0.133140 \\
  262144 &          356 &                     0.013661 &                      0.013691 &                            0.002214 &                 645158 &                     0 &         18.867962 &   64.0 &                        0.033710 &          0.645158 \\
 2097152 &          356 &                     0.013684 &                      0.013691 &                            0.000519 &                4907911 &                     0 &         18.867962 &  128.0 &                        0.032069 &          4.907911 \\
    4096 &         1824 &                     0.014018 &                      0.014050 &                            0.002261 &                 241948 &                     2 &         42.708313 &   16.0 &                        0.008396 &          0.241948 \\
   32768 &         1824 &                     0.014019 &                      0.014050 &                            0.002231 &                 287718 &                     1 &         42.708313 &   32.0 &                        0.008366 &          0.287718 \\
  262144 &         1824 &                     0.014021 &                      0.014050 &                            0.002053 &                 800978 &                     0 &         42.708313 &   64.0 &                        0.008189 &          0.800978 \\
 2097152 &         1824 &                     0.014043 &                      0.014050 &                            0.000517 &                5165856 &                     0 &         42.708313 &  128.0 &                        0.006663 &          5.165856 \\
    4096 &         7132 &                     0.014107 &                      0.014115 &                            0.000560 &                 936609 &                     3 &         84.451169 &   16.0 &                        0.002118 &          0.936609 \\
   32768 &         7132 &                     0.014107 &                      0.014115 &                            0.000545 &                 980583 &                     2 &         84.451169 &   32.0 &                        0.002102 &          0.980583 \\
  262144 &         7132 &                     0.014107 &                      0.014115 &                            0.000555 &                1469094 &                     1 &         84.451169 &   64.0 &                        0.002112 &          1.469094 \\
 2097152 &         7132 &                     0.014108 &                      0.014115 &                            0.000516 &                5745181 &                     0 &         84.451169 &  128.0 &                        0.002074 &          5.745181 \\
    4096 &        28160 &                     0.014130 &                      0.014132 &                            0.000140 &                3693308 &                     4 &        167.809416 &   16.0 &                        0.000533 &          3.693308 \\
   32768 &        28160 &                     0.014130 &                      0.014132 &                            0.000137 &                3684480 &                     4 &        167.809416 &   32.0 &                        0.000530 &          3.684480 \\
  262144 &        28160 &                     0.014130 &                      0.014132 &                            0.000138 &                4284185 &                     3 &        167.809416 &   64.0 &                        0.000531 &          4.284185 \\
 2097152 &        28160 &                     0.014130 &                      0.014132 &                            0.000139 &                8546585 &                     1 &        167.809416 &  128.0 &                        0.000532 &          8.546585 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-refinement-equidistant_sphere-SMCA.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  MAX\_REFINEMENT\_LEVEL &  N\_TRIANGLES\_ROOT &   N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &       167706 &                     0.013638 &                      0.014136 &                            0.035235 &                3115139 &                     0 &         409.51923 &  16.0 &                        0.035299 &          3.115139 \\
    4096 &       167706 &                     0.014009 &                      0.014136 &                            0.009033 &                6030219 &                     1 &         409.51923 &  16.0 &                        0.009099 &          6.030219 \\
    4096 &       167706 &                     0.014104 &                      0.014136 &                            0.002297 &                6570549 &                     2 &         409.51923 &  16.0 &                        0.002363 &          6.570549 \\
    4096 &       167706 &                     0.014128 &                      0.014136 &                            0.000581 &                7948544 &                     3 &         409.51923 &  16.0 &                        0.000647 &          7.948544 \\
\bottomrule
\end{tabular}


==> data/Data_Pandas_Dframe-refinement-perturbed_alpha_0.25_sphere-SMCA.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
 N\_CELLS &  N\_TRIANGLES &  VOLUME\_FROM\_VOLUME\_FRACTION &  VOLUME\_FROM\_SURFACE\_INTEGRAL &  VOLUME\_ERROR\_FROM\_SURFACE\_INTEGRAL &  CPU\_TIME\_MICROSECONDS &  MAX\_REFINEMENT\_LEVEL &  N\_TRIANGLES\_ROOT &   N\_C &  VOLUME\_ERROR\_FROM\_EXACT\_VOLUME &  CPU\_TIME\_SECONDS \\
\midrule
    4096 &       167706 &                     0.013642 &                      0.014136 &                            0.034938 &                3294823 &                     0 &         409.51923 &  16.0 &                        0.035002 &          3.294823 \\
    4096 &       167706 &                     0.014009 &                      0.014136 &                            0.008981 &                6539574 &                     1 &         409.51923 &  16.0 &                        0.009046 &          6.539574 \\
    4096 &       167706 &                     0.014104 &                      0.014136 &                            0.002257 &                7058193 &                     2 &         409.51923 &  16.0 &                        0.002323 &          7.058193 \\
    4096 &       167706 &                     0.014128 &                      0.014136 &                            0.000562 &                8301452 &                     3 &         409.51923 &  16.0 &                        0.000627 &          8.301452 \\
\bottomrule
\end{tabular}


==> figures/architecture-lichtenberg.tex <==
\begin{tabular}{lllll}
\toprule
Computing architecture A1 (Lichtenberg Cluster)& \\
\midrule
CPU \\         
  & vendor\_id	: GenuineIntel \\
  & cpu family	: 6\\
  & model	: 63 \\
  & model name	: Intel(R) Xeon(R) CPU E5-2680 v3 @ 2.50GHz \\
Compiler \\
  & version : g++ 9.1.0 \\
  & optimization flags : -std=c++2a -O3 \\
\bottomrule
\end{tabular}



==> research-highlights.tex <==
\section*{Highlights}

%address a problem of contemporary interest in physics that cannot be solved by current software are particularly encouraged.

%mathematical and numerical methods and algorithms;

%computational models including those associated with the design, control and analysis of experiments; and

%algebraic computation.

\begin{itemize}
    \item Computation of volume fractions on unstructured meshes from triangulated surfaces.
    \item Surfaces may have sharp edges and be composed of disjoint parts, e.g. from 3D scans.
    \item Accurate and second-order convergent results. 
    \item Efficient calculation of signed distances and inside/outside information.
\end{itemize}


==> response-to-reviewers/R0/sections/reviewer-1.tex <==
\noindent\emph{"Quote from the reviewer"}
\medskip

Our reply.

\noindent\emph{"Quote from the reviewer"}
\medskip

Our reply.


==> sections/backupfile-ahn-shashkov.tex <==
%
\begin{equation}
  \InterfaceCells = \{c : \exists (\vec{p},\vec{q}) \in \Cell_c, \vec{p} \text{ inside } \InterfaceMesh, \vec{q} \text{ not inside } \InterfaceMesh \},
  \label{eqn:mof:icells}
\end{equation}
\todo[inline]{the condition above strongly depends on what you consider $\Cell_c$ to be. if it is the set of corner points of the cell, this not generally a good definition (imagine a cell whose points are all located on a sphere. the cell is fully contained in the sphere, but not part of the set above. if  $\Cell_c$ is a subset of Rn, then the condition on $\vec{q}$ is unnessessary} 
\todo[inline]{what is the $i$ in the exponent of N?, $\Gamma_h$ is not properly defined yet. Is it supposed to be a set of points or the set of of points of the discrete interface or the points from which we built the interface?}
%
where $\vec{p}$ and $\vec{q}$ are points of the cell $\Cell_c$. Different algorithms have been developed to test if $\vec{p} \text{ inside } \InterfaceMesh$ that are of practical use for large values of $|\InterfaceMesh|,|\Domain|$. To ensure short calculation times on $3D$ unstructured meshes with large initial interfaces, \citet{Ahn2007jcp} relied on the \emph{ray crossing} version of a \emph{point-in-polyhedron} algorithm described by \citet[section 7.5]{ORourke1998} to compute $\vec{p} \text{ inside } \InterfaceMesh$.  To substantiate the decision for altering the initialization algorithm proposed by \citet{Ahn2007jcp,Ahn2007}, the ray crossing point-in-polyhedron algorithm of \citet{ORourke1998} is outlined in \cref{alg:gvof:raycross}. \todo[inline]{what is the goal of this sub-algorithm? for a single given cell to compute whether it is intersected?} 

\begin{algorithm}[]
    \centering
    \caption{Ray crossing point-in-polyhedron by \cite{ORourke1998}}
    \label{alg:gvof:raycross}
    {\small
      \begin{algorithmic}[1]
       \While{true} \textcolor{red}{for each q in ...?}
        \State compute bounding radius $R$ \textcolor{red}{bounding what? or is this a comment?}
        \State $\vec{r}_0=$ random ray of length $R$ \textcolor{red}{with random direction? or is this a random $\vec{r}_0 \in B_1(0)$}
        \State $\vec{r}=\vec{q} + \vec{r_0}$ \textcolor{red}{which \vec{q} is this?} 
        \State crossings $=0$
        \For{triangle $\Triangle \in \InterfaceMesh$}
          \Call{intersect}{$\Triangle,\vec{q},\vec{r}$} 
          \If{degenerate intersection} \textcolor{red}{what is a degenerate intersection?}
            \State re-enter while loop
          \Else 
            \State increment crossings  \textcolor{red}{crossings += 1?}
          \EndIf
        \EndFor
        \If{crossings is odd}
          \State \textbf{return} $\vec{q} \text{ is inside } \InterfaceMesh$
        \Else 
          \State \textbf{return} $\vec{q} \text{ not inside } \InterfaceMesh$
        \EndIf 
       \EndWhile
      \end{algorithmic}
    }
\end{algorithm}

\citet{ORourke1998} states that \cref{alg:gvof:raycross} is of complexity $\Oh(cn)$, where $c$ is the number of times the \texttt{while} loop has been re-entered to disregard a special case, and $n = |\InterfaceMesh|$. Experiments show that $\overline{c} \approx 1$, which makes \cref{alg:gvof:raycross} linear in terms of the size of the interface mesh $n=|\InterfaceMesh|$.\todo[inline]{if c is a constant, then the complexity is O(n) no matter what value c has} \todo[inline]{where can these experimental results be found?}
\todo[inline]{ToDo: the symbol $\Points$ has not been introduced yet (TT), what is this symbol denoting?}
If \cref{alg:gvof:raycross} is used to categorize all points of the domain $\Domain$ to identify interface cells $\InterfaceCells$ using \cref{eqn:mof:icells}, the overall complexity of evaluating $\InterfaceCells$ is of quadratic complexity $\Oh(mn)$ where $m = |\Points|$ and $n = |\InterfaceMesh|$. 


%
\begin{algorithm}[]
    \centering
    \caption{Volume fraction initialization : \cite{Ahn2007}}
    \label{alg:mof:vof}
    {\small
      \begin{algorithmic}[1]
        \For{cell c $\in \InterfaceCells$}
          \State AABBc = axis aligned bounding box (c) 
          \State compute random points $\Point$, $\Points_{AABBc} = \{ \Point : \Point \in AABB(c)\}$
          \State $n_{c}^p = |\Points_{AABBc}|$
          \State $n_{obj}^p = 0$
          \For{point $\Point \in \Points_{AABBc}$}
            \If{$\Point \text{ is inside } \InterfaceMesh$} 
              \State $n_{obj}^p = n_{obj}^p + 1$ 
            \EndIf
          \EndFor
        \State $\PlicFraction = \dfrac{n_{obj}^p}{n_c^p}$
        \EndFor
      \end{algorithmic}
    }
\end{algorithm}
%
\todo[inline]{type setting of AABB, what does the index "obj" mean?, $\Point \text{ is inside } \InterfaceMesh$ is misleading if you mean that the point is on one side of the interface,  "inside" requires an orientation of the interface which is not addressed so far, overall there are two sources of errors 1. the cell is approximated via a bounding box and 2. choosing random points.}

For interface cells $\InterfaceCells$ identified by \cref{alg:gvof:raycross}, \citet{Ahn2007} compute the volume fraction using \cref{alg:mof:vof}. Two important conclusions can be drawn by examining \cref{alg:mof:vof}. First, the computation of the volume fraction $\PlicFraction$ is approximative, as it is defined by the ratio of the number of points inside $\InterfaceMesh$ and the total number of points that fill \emph{the axis-aligned bounding box of an interface cell} $c \in \InterfaceCells$, compared to using geometrical intersections to compute $\Cell_c \cap \InterfaceMesh$. Therefore, the accuracy of \cref{alg:mof:vof} depends on the number of points randomly distributed within the bounding box of the interface cell $n_c^p$. Moreover, using the points that fill an axis aligned bounding box of a cell to compute its volume fraction is an inaccurate representation of the volume fraction on tetrahedral meshes \todo{but basically on every polyhedral cell and even on hex-meshes that are not axis aligned, right?}, where the axis aligned bounding box may differ strongly from the geometry of the tetrahedron (cf. \cref{fig:mof:init}). This error is avoided when hexahedral cells are used to discretize the domain $\Domain$ and is lower for polyhedral cells. Second, \cref{alg:mof:vof} has the complexity of $\Oh(|\InterfaceCells| n_c^p |\InterfaceMesh|)$ when it comes to categorizing each point $\Point \in \Points_{AABBc}$ using the ray crossing algorithm. 

\begin{figure}[htb] 
   \begin{center}
    \def\svgwidth{0.6\textwidth}
     {\footnotesize
        \input{figures/cylinder2DmeshInit.pdf_tex}
     }
   \end{center}
    \caption{Schematic representation of the volume fraction initialization
    algorithm of \cite{Ahn2007}. The randomly generated points are
    schematically shown as circles of different colors: those that are inside
    $\InterfaceMesh$ are of white color and they contribute to $n_{obj}^p$ in
    \cref{alg:mof:vof}. Obviously in this schematic case, all the points that
    are inside $\InterfaceMesh$ are not inside the triangular cell $\Cell_c$; however
    they are used to compute $\PlicFraction$.} 

    \label{fig:mof:init}
\end{figure}

The number $n_c^p$ can be considered a large constant in this case, as surely more than $10$ points are required to accurately represent the fill level of the cell bounding box. Consequently, the total complexity of the algorithm proposed by \cite{Ahn2007} to compute the volume fraction is $Oh((|\Domain| + |\InterfaceCells| n_c^p) |\InterfaceMesh|)$ - if the complexity is analyzed in terms of the intersection between a triangle and a ray. As stated by \cite{Ahn2007}, $n_c^p$ is a small number compared to $|\Domain|$, however, it is multiplied with $n_c^p$ which can be large \todo{sentence makes no sense? where is $n_c^p$multiplied by itself?}. Of course, this is the worst case complexity, since the ray-triangle intersection can be avoided by introducing AABB tests as proposed by \cite{ORourke1998} \todo{so Anh2007 has the bounding box/stochastic approach from O'Rourke?}. The initialization algorithm \cref{alg:mof:vof} requires additional bounding box tests to include cells of $\Domain$ into $\InterfaceCells$ that cannot be identified by \cref{alg:gvof:raycross} because their size may be too large to resolve small features of $\InterfaceMesh$.  However, this difference is ignored in this description of new initialization algorithms as sufficiently resolved meshes are used.



==> sections/cci-old-backup.tex <==

Two reasons exist for changing the outlined volume fraction calculation algorithms on unstructured meshes:  obtaining an exact volume fraction field and a need for a more efficient inside-outside point categorization. In order to achieve this, the volume fraction is computed using geometrical intersections
%
\begin{equation}
  \PlicFraction = \dfrac{\text{volume}(\Cell_c \cap \InterfaceAppr)}{V_c},
  \label{eqn:gvof:alpha-inter}
\end{equation}
%
where $V_c$ is the volume of the cell $\Cell_c$. Two algorithms are developed that rely on \cref{eqn:gvof:alpha-inter} for exact calculation of the volume fraction: the Cell - Cell Intersection (CCI) algorithm (a slightly modified algorithm of \citet{Ahn2007}) and new the Surface Mesh - Cell Intersection (SMCI) algorithm, outlined in respective \cref{alg:gvof:cci,alg:gvof:smci}. 

%
\begin{algorithm}[]
    \centering
    \caption{CCI volume fraction initialization} 
    \label{alg:gvof:cci}
    {\small
      \begin{algorithmic}[1]
        \State Compute $B_\Omega : \{B_\Omega^i: B_\Omega^i = \text{ AABB}(\Cell_i), \Cell_i \in \Domain \}$ 
        \State Compute $B_\Gamma : \{B_\Gamma^j: B_\Gamma^j = \text{ AABB}(\Triangle_i), \Triangle_i \in \InterfaceAppr \}$ 
        \State $B_{\Omega,\Gamma} = \{B_{\Omega,\Gamma}^i : B_{\Omega,\Gamma}^i =  \emptyset$ \}
        \For{$i \in [1,|B_\Omega|]$}
          \For{$j \in [1,|B_\Gamma|]$}
            \If {$B_\Omega^i  \cap B_\Gamma^j \ne \emptyset$}
              \State $B_{\Omega,\Gamma}^i = B_{\Omega,\Gamma}^i \cup j$
            \EndIf
          \EndFor
        \EndFor
        \For{$B_{\Omega,\Gamma}^i \in B_{\Omega,\Gamma}$}
          \State $V_{\alpha,c} = 0$
          \For{$j \in B_{\Omega,\Gamma}^i$} 
            \State $V_{\alpha,c} += \text{volume}(\Cell_i \cap \Cell_j), \Cell_i \in \Domain, \Cell_j \in \InterfaceAppr$
          \EndFor 
          \State $\PlicFraction = \dfrac{V_{\alpha,c}}{V_c}$
        \EndFor 
      \end{algorithmic}
    }
\end{algorithm}
%

CCI \cref{alg:gvof:cci} is a step in the right direction of computing an exact $\PlicFraction$ value. However, it has a complexity of $\Oh(|\Domain|\overline{d})$ in terms of the $3D$ polyhedron intersection operation which costs much more than the triangle / ray intersection utilised by \cref{alg:mof:vof}. The number $\overline{d}$ is the average number of cells $\Cell_j \in \InterfaceAppr$ that intersect a cell $\Cell_i \in \Domain$. This number depends on the relative size of the cells in $\Domain$ compared to the cells in $\InterfaceAppr$: it grows when the size of the cells in $\InterfaceAppr$ is reduced. The first part of the algorithm reduces the complexity from $\Oh(mn)$ where $m = |\Domain|$ and $n = |\InterfaceAppr|$, by pre-computing AABBs of cells in $\Domain$ and $\InterfaceAppr$, which is a very cost-effective operation. In order to keep $\overline{d}$ as small as possible, $\InterfaceAppr$ mesh is created as an unstructured mesh, refined near its boundary that represents the fluid interface. This way, the complexity of the algorithm is reformulated as $\Oh(k|N_b| + l|\InterfaceCells|)$, where $N_b = \{ \Cell_c : \Cell_c \in \Domain, \alpha_c = 1 \}$, with $\overline{k} \approx 10$, $\overline{l} \approx 100$ and of course $|\InterfaceCells| << |\InterfaceAppr| << |\Omega|$. This reduction in effect makes \cref{alg:gvof:cci} have linear complexity with respect to the cell/cell intersection operation. Because the initial interface mesh $\InterfaceAppr$ is used for initializing the volume fraction field, a strong non-uniform refinement near the fluid interface boundary of $\InterfaceAppr$ can be applied. With $k=100$ in interface cells, the initial interface is approximated with $100$ cells of $\InterfaceAppr$ within a single cell $\Cell_i \in \Domain$. 

The proposed reduction in complexity of the CCI algorithm can be described graphically. Consider the uniformly refined initial interface mesh $\InterfaceAppr$ shown in \cref{fig:cylinder2Dmesh}. A local refinement near the interface can be used on $\InterfaceAppr$ to increase the volume fraction calculation accuracy, as shown in \cref{fig:interfaceMeshRefined}. The initial interface mesh $\InterfaceAppr$ that is refined near the interface ensures sufficient interface resolution for an accurate $\PlicFraction$ value. Very coarse cells away from the interface reduce the algorithm complexity, as the internal cells of $\Domain$ are intersected with but a few cells of the interface mesh $\InterfaceAppr$. \Cref{fig:gvof:cci} contains geometrical results from an actual algorithm execution. It is clearly visible that the volume fraction computation $\PlicFraction = \frac{\text{volume}(\InterfaceAppr \cap \, \Cell_c)}{V_c}$ in the case of the CCI algorithm involves many cell / cell intersections ($\Cell_i \cap \Cell_j$ in \cref{alg:gvof:cci}) for interface cells (cell $\Cell_c$ in \cref{fig:gvof:cci}), in order to ensure that the interface $\InterfaceAppr$ is sufficiently resolved.

\begin{figure}[htb] 
  \centering
  \subfloat[Local refinement of the interface mesh $\InterfaceAppr$.]{
    \label{fig:interfaceMeshRefined}
    \centering
    \def\svgwidth{0.4\columnwidth}
    \centering
     {\footnotesize
        \input{figures/cci-algorithm-input.pdf_tex}
     }
   }
  \subfloat[Visualization of the intersection $\Cell_c \cap \InterfaceAppr$.]
  {
    \centering
    \def\svgwidth{0.4\columnwidth}
    \centering
     {\footnotesize
        \input{figures/cci-algorithm-output.pdf_tex}
     }
  } 

  %\caption{Volume fraction initialization of a verification case using the CCI algorithm. The interface $\InterfaceAppr$ is modeled as an unstructured volume mesh. The exact volume fraction value $\PlicFraction$ is computed using $\Cell_c \cap \InterfaceAppr$. left image shows an overlay of $\InterfaceAppr$ and a cell $\Cell_c$, and the right image contains the actual result of a geometrical intersection $\InterfaceAppr \cap \Cell_c$.} 

  %\label{fig:gvof:cci}
%\end{figure}

%The CCI \cref{alg:gvof:cci} computes exact volume fractions, and is amenable to multiple phases, by using multiple initial interface meshes $\InterfaceAppr$. It is however very important to note that the linear complexity of \cref{alg:gvof:cci} cannot be compared to the quadratic complexity of \cref{alg:mof:vof}, for the obvious difference in the \emph{unit operation}: the operation used to analyze the complexity of the algorithms. The unit operation is usually that operation where the majority of the computational time is spent by the algorithm. In asymptotic complexity analysis, algorithm operations are often assumed to take the same amount of time, which is a false and dangerous way of analyzing algorithmic complexity, especially with large problems characteristic to CFD. In this work, a unit operation is isolated using profiling tests with many problem sets of increased sizes. CCI algorithm was not implemented for its low complexity or execution times, the main goal was to ensure exact volume fraction initialization. 

%Another significant source of the computatioal complexity of the CCI algorithm comes from the intersections of the all the bulk cells $\PlicFraction = 1$ with the interface mesh $\InterfaceAppr$. Because those cells are filled completely, no intersections should be performed in order to set their volume fraction values $\PlicFraction = 1$. Since the cells with $\PlicFraction = 1$ are filled with phase $1$, the costly cell / cell intersection could be replaced by an algorithm that marks them as \emph{inside cells} or \emph{bulk cells}. For this purpose, the new Surface Mesh Cell Intersection (SMCI) algorithm (outlined in \cref{alg:gvof:smci}) is proposed that performs a fast inside-outside categorization using spatial sub-divison based on the octree data structure that supports fast search queries (\citet{Meagher1982,Mehta2004}) within a narrow band of cells that surround the interface. The sign of the distance is then propagated for the bulk cells by solving a diffusion equation for the distance.


==> sections/results-bunny.tex <==
\subsection{Stanford bunny} 
\label{subsec:bunny}


==> sections/results-old.tex <==
% TODO: Old text, remove
%Box plots are reported for statistical data with $90\%$ confidence intervals. If not otherwise stated, mean values are computed over $1000$ repeated calculations with a uniformly randomized input: a random position of the tool-mesh bounding box is computed within the base-mesh bounding box for each intersection test. 

%The parameters used in the verification process are shown in \cref{tab:verification}. 

%\begin{table}[!htb]
  %\begin{center}
      %{\footnotesize
        %\input{tables/verification-parameter-table.tex}
      %}
  %\end{center}
  %\caption{Verification parameters.}
  %\label{tab:verification}
%\end{table}

%%\begin{equation}
  %%N_{t,b} = |\Omega_{t,b}|
%%\end{equation}

%The volume conservation error of the SMCI and CCMI algorithms is defined as the absolute difference between the total volume of the tool-mesh computed from its volume fraction on the base-mesh, and the tool-mesh volume given by its geometry,  
%\begin{equation}
  %E{v} = \dfrac{|\sum_{c=1}^{|\Omega_b|}\alpha_c V_c - \sum_{d=1}^{|\Omega_t|}V_d|}{\sum_{e=1}^{|\Omega_t|} V_e}.
%\end{equation}

%Initialization time $T_i$ is the time required to initialize the input data used by the algorithms. This time is reported in order to compare the computation time with the initialization time: a usable initialization of the volume fraction field should require less time than what is needed to initialize the required input data.  

%The execution time $T_e$ represents the time needed to perform the calculations necessary for initializing the volume fraction field. Reported total number of cell / halfspace intersections $N_x$ confirms its detrimental impact on the computational efficiency of both algorithms, as described in \cref{sec:alphainit}. The number of interface cells $N_i$ approximately corresponds to the number of intersected cells for the SMCI algorithm, because a bounding box of an arbitrary cell may intersect a bounding box of a set of triangles, in such a way that their intersection has zero volume. The number of bulk cells $N_k$ is important for the CCMI algorithm, as those cells are intersected by the CCMI algorithm. Bukl intersections are avoided by the bulk identification part of the SMCI algorithm that relies on sign propagation. 

%\subsection{Cylindrical interface} 
%\label{sec:cylinder}

%\begin{figure}[htb] 
    %\centering
    %\subfloat[SMCI cylindrical interface.]{
        %\centering
        %\includegraphics[width=0.3\textwidth]{figures/SMCI-input-cylinder.png}
        %\label{fig:cylinput:smci}
    %}
    %\subfloat[CCMI cylindrical interface.]{
        %\centering
        %\includegraphics[width=0.3\textwidth]{figures/CCMI-input-cylinder.png}
        %\label{fig:cylinput:ccmi}
    %}
    %\caption{Cylindrical tool-meshes used by the SMCI and CCMI algorithms.}
    %\label{fig:cylinput}
%\end{figure}


%The SMCI and CCMI algorithms are implemented in $3D$, so the $2D$ calculations are performed on a prismatic layer of $3D$ mesh cells. In order to investigate the efficiency and accuracy of both algorithms, a cylindrical tool-mesh is intersected with the base-mesh. The surface mesh used by the SMCI algorithm and the volume mesh used by the CCMI algorithm are shown in \cref{fig:cylinput}. The cylinder has a radius $R_c = 0.15$ and is placed randomly within a domain of dimensions $[1 \times 1 \times 0.1]$. The surface tool-mesh shown in \cref{fig:cylinput:smci} is produced by dividing the circumference of the cylinder in $512$ intervals, that result in $512$ rectangles with a cylinder height $0.1$, that are then diagonally split into triangles. The volume tool-mesh used by the CCMI algorithm shown in \cref{fig:cylinput:ccmi} is generated using the surface cylinder mesh shown in \cref{fig:cylinput:smci} with a matching mesh resolution used to approximate the interface. An automatic unstructured mesh generation algorithm is used with a local mesh refinement near the cylindrical interface and a strongly decreased mesh resolution in the bulk with the goal of reducing the number of intersections in the bulk for the CCMI algorithm. Any unstructured mesh generation algorithm that supports local mesh refinement can be used for this purpose. The \emph{cartesian2D} algorithm from the Open Source \emph{cfMesh} meshing software was used in this study. The mesh generation parameters used for the tool-mesh are available in the data repository. 

%\begin{figure}[htb] 
    %\centering
    %\subfloat[Volume error $E_v$ of the SMCI algorithm.]{
        %\centering
        %\includegraphics[]{figures/SMCIEv.pdf}
        %\label{fig:ev:smci}
    %}
    %\subfloat[Volume error $E_v$ of the CCMI algorithm.]{
        %\centering
        %\includegraphics[]{figures/CCMIEv.pdf}
        %\label{fig:ev:ccmi}
    %}
    %\label{fig:ev}
    %\caption{Volume errors of SMCI and CCMI algorithms.}
%\end{figure}

%Box-plots of the volume error $E_v$ are shown in \cref{fig:ev:smci,fig:ev:ccmi}, for the respective SMCI and CCMI algorithm across all mesh resolutions. Both SMCI and CCMI algorithms show a stable error distribution with a few outlying cases where the $E_v$ approaches machine tolerance, for cases with very low mesh resolution. The geometrical intersection between a halfspace and a polyhedron used by the CCMI and SMCI algoirthm is relying on tolerance-based logic to deal with coplanarity, collinearity and coincidence. Tolerance-based logic results in an increase of the computational efficiency at the cost of accuracy \citet[ch. 11]{Ericson2004}. Calculation of the $E_v$ near machine-tolerance is not possible with the tolerance-based intersection logic, for the intersection configurations required by the VoF initialization. Both SMCI and CCMI algorithms require multiple intersections that involve exact coplanarity and coincidence. A subset of triangles that is used to intersect a cell by the SMCI algorithm contains edge-adjacent triangles. The CCMI algorithm likewise requires intersections between an interface cell and a subset of cells where some cells are face-adjacent. Once a first intersection is computed with an interface cell with either algorithm, intersection points computed with the will contain a numerical roundoff error. Any subsequent intersection that involves coplanarity results either in another roundoff error if the previous intersection caused the common point to be placed outside of the tolerance interval, or in a projection of the point onto the plane, which obviously also changes its position. These slight differences in point positions for points that are actually unique results in the slight difference in the volume of the computed cell intersection. As there is no reason to expect that those errors cancel out, the total $E_v$ error is expected to increase with the total number of intersections, which is shown in \cref{fig:ev:ccmi} and \cref{fig:ev:smci}. 

%\begin{figure}[htb] 
    %\centering
    %\subfloat[Text]{
        %\centering
        %\includegraphics[]{figures/SMCITe.pdf}
    %}
    %\subfloat[Text]{
        %\centering
        %\includegraphics[]{figures/CCMITe.pdf}
    %}
    %\label{fig:smciev}
    %\caption{Description.}
%\end{figure}

%\begin{table}[!htb]
  %\begin{center}
      %{\footnotesize
        %\input{tables/SMCImean.tex}
      %}
  %\end{center}
  %\caption{SMCI mean data table.}
  %\label{tab:smci:mean}
%\end{table}

%\begin{table}[!htb]
  %\begin{center}
      %{\footnotesize
        %\input{tables/CCMImean.tex}
      %}
  %\end{center}
  %\caption{CCMI mean data table.}
  %\label{tab:smci:mean}
%\end{table}

%\begin{figure}[htb] 
    %\centering
    %\subfloat[Text]{
        %\centering
        %\includegraphics[]{figures/TeNx.pdf}
    %}
    %\subfloat[Text]{
        %\centering
        %\includegraphics[]{figures/TeNbLogLog.pdf}
    %}
    %\newline
    %\subfloat[Text]{
        %\centering
        %\includegraphics[]{figures/TeRatioNb.pdf}
    %}
    %\subfloat[Text]{
        %\centering
        %\includegraphics[]{figures/NxNb.pdf}
    %}
    %%
    %\label{fig:tenb}
    %\caption{Description.}
%\end{figure}


%\subsection{Spherical interface} 
%\label{sec:sphere}

%\todo[inline]{Run 3D cases with different meshes and comment on impossible computation times for the CCI algorithm} 

%\subsection{Stanford bunny} 
%\label{sec:bunny}

%\section{Application - Capillary Bridges on Hydrophobic Stripes}

%\begin{figure}[H] 
    %\centering
    %\subfloat[Minimal surface from Surface Evolver.]{
        %\centering
        %\includegraphics[height=0.36\textwidth]{figures/surfaceEvolver_init.pdf}
        %\label{fig:surface_evolver}
    %}
    %\subfloat[Comparison between physical interface and initial VOF-interface.]{
        %\centering
        %\includegraphics[height=0.36\textwidth]{figures/dropBreakup.png}
        %\label{fig:drop_exp_to_sim}
    %}
    %%
    %\label{fig:breakup}
    %\caption{Initialization for the intitial interface shape for a drop-breakup case, adapted from \cite{Hartmann2019}.}
%\end{figure}

%\begin{figure}[H] 
    %\centering
    %\subfloat[]{
        %\centering
        %\includegraphics[height=0.32\textwidth]{figures/breakup_crude.png}
        %\label{fig:breakup_crude}
    %}
    %\subfloat[]{
        %\centering
        %\includegraphics[height=0.32\textwidth]{figures/breakup_good.png}
        %\label{fig:breakup_good}
    %}
    %%
    %\label{fig:breakup_init}
    %\caption{Comparison of initial geometries.}
    %\todo[inline]{Mathis is looking for the "bad" simulations results based on the crude initial data. this will further illustrate the relevance. should we put this here?} 
%\end{figure}

%\newcommand{\thetaPhil}{\ensuremath{\theta_\text{phil}}}
%\newcommand{\thetaPhob}{\ensuremath{\theta_\text{phob}}}

%The algorithms described in Section \todo{add ref} has been applied in \cite{Hartmann2019} to obtain highly accurate initial data for the simulation of the breakup dynamics of a liquid drop on a patterned surface. The overall setup is illustrated in \cref{fig:surface_evolver}. The line where the liquid-gas interface intersects with the solid is the \emph{contact line}. The angle that is enclosed between the interface and the solid is called \emph{contact angle} and is  measured through the liquid. For the setup illustrated in \cref{fig:surface_evolver}, the solid surface has been coated with parallel hydrophilic and hydrophobic stripes, leading to different contact angles of $\thetaPhil=\SI{}{\degree}$ and $\thetaPhob = \SI{}{\degree}$, respectively \todo{add angles}. A liquid drop that is placed onto the coated surface immediately deforms into the shape shown in \cref{fig:surface_evolver} and the top of \cref{fig:drop_exp_to_sim}. 

%Initially, the drop is placed into a vapor-saturated atmosphere, where a volume change due to evaporation is negligible. This gives a reproducable and long-time stable initial condition. Then, the vapor concentration is decreased and the drop begins to evaporate, leading to a reduction of the bridge diamter $d$ and finally a breakup of the liquid bridge on the hydrophobic stripe. To analyze the drop breakup using numerical simulations, a highly accurate initial interface shape is essential for the correct predicton of the breakup dynamics. 

%In the stationary state, the shape of the liquid-gas interface is a minimal surface. To compute such a minnimal surface for the setup described above, the drop volume, the shape of the contact line, and the contact angles $\thetaPhil$ and $\thetaPhob$ are required and can be obtained by experimental measurements. In a first step, this input data is used to computed the minimal surface illustrated in \cref{fig:surface_evolver} using the computational tool Surface Evolver \cite{Brakke1992}. Surface Evolver computes a triangulated surface by minimizing a free energy functional subject to a prescribed volume. The computed interface is given using the Standard Triangulation Language (STL). The algorithm \todo{add ref} has been used to transform this surface description into a discrete indicator function such as \cref{eqn:volfrac-initial-func} that can be used in a VOF simulation. This fraction field has been used as initial conditions for a numerical simulation by a  geometric VOF approach. The interface that has been reconstructed based on the transformed STL-data is shown in the lower part of  \cref{fig:drop_exp_to_sim}, where an excellent agreeemnt with the experimentally observed interface can be seen. For a more detailed description of the involved procedure and results for the drop breakup dynamics see \cite{Hartmann2019}.


==> significance-and-novelties.tex <==
\section*{Significance and novelty}

%address a problem of contemporary interest in physics that cannot be solved by current software are particularly encouraged.

%mathematical and numerical methods and algorithms;

%computational models including those associated with the design, control and analysis of experiments; and

%algebraic computation.

Successful simulations of surface tension-driven two-phase flows using the unstructured Volume-of-Fluid (VOF) method (cf. \citep{Maric2020vofrev} for a recent review) depend on the accurate calculation of volume fractions. 
Erroneous initialization of volume fractions \textcolor{Reviewer1}{can lead to critical instabilities} since the VOF initialization errors significantly amplify curvature errors \citep{Kromer2019}.
Existing contributions address this problem \citep{Bna2015, Ivey2015, Bna2016, Strobl2016, Fries2016, Lopez2019, Kromer2019} by modeling fluid interfaces using functions and combining higher-order quadratures with mesh adaptivity to ensure accuracy.
Our numerical method significantly extends existing contributions in terms of the admissible shape of the fluid interface. 
Such surfaces can be composed of disjoint parts, and they can be closed or open, admitting very complex shapes and configurations.
We have recently successfully used the proposed methodology for initializing simulations of experiments involving the breakup dynamics of capillary bridges on hydrophobic stripes \citep{Hartmann2021}, which was not possible using other contemporary methods.
% Additionally, the proposed computationally efficient calculation of signed distances and inside-outside information (phase indication)   

% The numerical algorithms of the \texttt{triSurfaceImmersion} library are directly available as an OpenFOAM module and can be used within OpenFOAM. The resulting data can be converted into formats of other commercial and non-commercial CFD software. Alternatively, the proposed algorithms can be implemented in another software, provided an octree data structure and the ability to solve a Laplace equation are available. 


==> tables/CCMImean.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &   Nt &      Nb &       Ev &       Ti &       Te &     Nx &   Ni &    Nb.1 \\
N    &      &         &          &          &          &        &      &         \\
\midrule
2    & 2268 &       4 & 7.18e-14 & 2.58e-01 & 3.16e-02 &   2309 &    2 &       1 \\
4    & 2268 &      16 & 7.18e-14 & 1.96e-01 & 3.20e-02 &   2341 &    4 &      11 \\
8    & 2268 &      64 & 4.55e-09 & 1.64e-01 & 3.33e-02 &   2408 &    9 &      54 \\
16   & 2268 &     256 & 1.20e-08 & 3.75e-01 & 3.40e-02 &   2570 &   19 &     236 \\
32   & 2268 &    1024 & 1.67e-08 & 2.47e-01 & 4.38e-02 &   2909 &   38 &     985 \\
64   & 2268 &    4096 & 1.95e-08 & 2.02e-01 & 7.15e-02 &   3721 &   76 &    4019 \\
128  & 2268 &   16384 & 2.09e-08 & 5.73e-01 & 1.63e-01 &   5850 &  153 &   16230 \\
256  & 2268 &   65536 & 2.16e-08 & 1.03e+00 & 4.87e-01 &  12126 &  307 &   65229 \\
512  & 2268 &  262144 & 2.20e-08 & 2.31e+00 & 1.62e+00 &  32691 &  614 &  261529 \\
1024 & 2268 & 1048576 & 2.22e-08 & 9.35e+00 & 5.98e+00 & 106143 & 1228 & 1047347 \\
2048 & 2268 & 4194304 & 2.23e-08 & 3.00e+01 & 2.48e+01 & 381951 & 2457 & 4191846 \\
\bottomrule
\end{tabular}


==> tables/SMCImean.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
{} &   Nt &      Nb &       Ev &       Ti &       Te &       Tx &   Nx &   Ni &      Nk \\
N    &      &         &          &          &          &          &      &      &         \\
\midrule
2    & 1024 &       4 & 2.24e-08 & 2.45e-01 & 3.28e-01 & 3.27e-01 & 1027 &    2 &       2 \\
4    & 1024 &      16 & 2.24e-08 & 1.66e-01 & 1.66e-01 & 1.65e-01 & 1033 &    4 &      11 \\
8    & 1024 &      64 & 2.24e-08 & 1.69e-01 & 9.85e-02 & 9.68e-02 & 1042 &    9 &      54 \\
16   & 1024 &     256 & 2.24e-08 & 1.79e-01 & 6.80e-02 & 6.52e-02 & 1062 &   19 &     236 \\
32   & 1024 &    1024 & 2.24e-08 & 1.95e-01 & 6.37e-02 & 5.82e-02 & 1100 &   38 &     985 \\
64   & 1024 &    4096 & 2.24e-08 & 2.67e-01 & 7.33e-02 & 6.25e-02 & 1177 &   76 &    4019 \\
128  & 1024 &   16384 & 2.24e-08 & 5.48e-01 & 9.55e-02 & 7.69e-02 & 1331 &  153 &   16230 \\
256  & 1024 &   65536 & 2.24e-08 & 6.81e-01 & 1.81e-01 & 1.29e-01 & 1638 &  307 &   65228 \\
512  & 1024 &  262144 & 2.24e-08 & 2.73e+00 & 4.94e-01 & 3.06e-01 & 2252 &  614 &  261529 \\
1024 & 1024 & 1048576 & 2.24e-08 & 8.52e+00 & 1.61e+00 & 9.07e-01 & 3481 & 1228 & 1047347 \\
2048 & 1024 & 4194304 & 2.24e-08 & 2.87e+01 & 5.63e+00 & 2.99e+00 & 5939 & 2457 & 4191846 \\
\bottomrule
\end{tabular}


==> tables/verification-parameter-table.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
%{} &   Nt &      Nb &       Ev &       Ti &       Te &     Nx &   Ax &   Ni &    Nk \\
Parameter  &   Description \\
\midrule
$N_t$    &  Tool mesh size: number of cells (CCMI) or triangles (SMCI). \\
$N_b$    &  Number of base mesh cells. \\
$E_v$    &  Volume conservation error. \\
$T_i$    &  Initialization time. \\ 
$T_e$    &  Execution time. \\ 
$N_x$    &  Total number of cell / halfspace intersections. \\ 
$N_i$    &  Number of interface cells. \\ 
$N_k$    &  Number of bulk cells. \\ 
\bottomrule
\end{tabular}

